Evaluating LLMs for Targeted Concept Simplification for Domain-Specific Texts

One useful application of NLP models is to support people in reading complex text from unfamiliar domains (e.g., scientific articles). Simplifying the entire text makes it understandable but sometimes removes important details. On the contrary, helping adult readers understand difficult concepts in context can enhance their vocabulary and knowledge. In a preliminary human study, we first identify that lack of context and unfamiliarity with difficult concepts is a major reason for adult readers' difficulty with domain-specific text. We then introduce "targeted concept simplification," a simplification task for rewriting text to help readers comprehend text containing unfamiliar concepts. We also introduce WikiDomains, a new dataset of 22k definitions from 13 academic domains paired with a difficult concept within each definition. We benchmark the performance of open-source and commercial LLMs and a simple dictionary baseline on this task across human judgments of ease of understanding and meaning preservation. Interestingly, our human judges preferred explanations about the difficult concept more than simplification of the concept phrase. Further, no single model achieved superior performance across all quality dimensions, and automated metrics also show low correlations with human evaluations of concept simplification ($\sim0.2$), opening up rich avenues for research on personalized human reading comprehension support.

==> old_dump.tex <==
Facilitating comprehension of technical writing promotes learning and broader communication of ideas. Text simplification supports comprehension for students and new language learners by substituting complex terms and reducing complex syntax.
%Simplifying text by substituting complex terms and reducing complex syntax aids students and new language learners by reducing overall reading difficulty. 
However, text simplification also sacrifices intricate details and specific terminologies about concepts that are necessary for in-depth understanding of the subject. Alternatively, scaffolding readers with explanations for difficult concepts can enable richer in-context understanding of subjects. In this work, we propose a new task of supporting end-user concept difficulty

simplifying user specific difficult concepts in technical definitions through explanations or additional context. To evaluate our work, we introduce a dataset of definitions spanning ten high-level domains extracted from Wikipedia. We evaluate the performance of open-source and commercial LLMs to explain or expand on domain specific concepts and introduce a novel graph based metric to evaluate LLM generated definitions for concept explanations. We find that LLMs vary greatly in their manner of rewriting definitions to alleviate concept difficulty in terms of verbosity, and choice of terms. Automated evaluations and follow-up open-ended human feedback on difficulty with definitions suggests that users prefer addition context such as in-context explanations, examples or illustrations over simply reducing the reading level of text opening up new directions for simplification research in NLP.

% Do nlp systems preserve meaning - https://arxiv.org/abs/2312.10126
% BLESS: Benchmarking Large Language Models on Sentence Simplification - https://aclanthology.org/2023.emnlp-main.821.pdf
% Controlling pre-trained langauge models for grade specific text simplification - https://aclanthology.org/2023.emnlp-main.790.pdf
% Use reading difficulty in first line for coherence.

%Such lack of information can hinder them from learning about the domain, or communicating ideas. %We lack an understanding of how to effectively balance simplicity with the retention of domain-specific intricacies of concepts.

%Which leads to  \textit{Lexical}~\cite{devlin1999simplifying} and \textit{syntactic}~\cite{siddharthan2006syntactic} simplifications focus on XYZ, and datasets contains YZ. Such methods alleviate reading difficulty for new language learners, children, or a lay audience by substituting complex syntax or words with simpler alternatives or omitting difficult phrases altogether while preserving the broader meaning~\cite{}. However, coarse-grained simplification of an entire text also loses the richness of text~\cite{garbacea-etal-2021-explainable} as all the information is not necessary for a simplified version (see Figure~\ref{fig:text_difficulty_overview}). This can be detrimental in professional or educational scenarios where users may possess selective expertise of the domain and can benefit from specific explanations or simplifications in-context rather than removing information altogether~\cite{}.

% However, domain experts can often struggle to understand how to write documents for broader communication, or may simply not have the time to rewrite existing documents for a broader audience[]. 

% Computational models to address reading difficulty have focused on predicting reading difficulty and rewriting difficult text into simpler alternatives.
% NLP simplification methods can alleviate the problem of domain difficulty by automatically translating complex sentences into simpler versions that require less domain expertise. However simplification methods focus on difficult words or syntax difficulty replacing difficult words in  

% Current NLP methods have attempted simplification ranging from grade level treat simplification as a binary task of complex and simple sentences  Automated methods to simplify text can provide support in increasing accessibility of documents. where simpler text can be easy to understand for readers but at the expense of losing important information. 

%Grade based simplification methods are trained on grade-level or binary simplification corpus (Newsela, Zhang et al) and cannot perform targeted concept simplifications based on user's background and knowledge. 
% Large language models (LLMs) can rewrite text based on specific instructions to simplify text~\cite{}. However, LLMs can show a range of behavior in rewriting text to suit reader's difficulty ranging from substituting difficult concepts with simpler alternatives, or adding explanations for concepts. Even the instruction following capabilities of LLMs are under active research and it is unclear if LLMs can appropriately simplify text in-context for personalized difficulty~\cite{}.

%- 56.9% of Q1 mentioned complex concepts and 24.6% mentioned needing more context or additional detail.  9.2% mentioned needing simpler language from a syntax perspective.  About 8% mentioned needing exmaples or analogies and 8% wanted more visual/audio information (how does this look like; how would this be pronounced).   Smaller amounts of people said that the definition was too specific or redundant, too technical/formal, need clarification or just not a well-written definition.
%- 46% asked the "tutor" to explain or breakdown complex terms.  44% asked for more context or details to be added to the defiinition.  25% asked for examples, analogies.  Only 13% asked for a simpler syntax/phrasing
%We identified that X\% of definitions had some mention of difficulty associated with them. For the open-codes, the top-5 codes associated with definition difficulty were 1) XX, 2) XX, 3) XX, 4) XX, 5) XX. All of these codes suggest that participants had difficulty with the definitions due to the difficulty in integrating the concepts in the definition with their world knowledge.


% \begin{table*}[h]
%     \centering
%     \begin{tabular}{p{1.2cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1.1cm}|p{1.2cm}|p{1.2cm}|p{1.1cm}|p{1.1cm}}
%     \toprule
%         LLM & Dataset & Defin-itions & density & H-concept-\_max & H-meaning-\_preserve & H-rewrite-\_easier & H-rewrite-\_understand & H-familiar\\
%     \midrule
%         Bloomz  & enwiki & 120 & 11.65 & 0.38 & 4.20 & 0.32 & 0.54 & 2.60\\
%         Falcon & enwiki & 120 & 6.65 & 0.45 & 4.00 & 0.50 & 0.71 & 2.55\\
%         PaLM2 & enwiki & 120 & \textbf{19.35} & 0.42 & \textbf{4.43} & 0.29 & 0.58 & 2.59\\
%         GPT4 & enwiki & 120 & 4.68 & \textbf{0.57} & 4.24 & \textbf{0.56} & \textbf{0.79} & 2.70\\
%         \midrule
%         Bloomz & scidef & 60 & 12.80 & 0.39 & 4.22 & 0.39 & 0.56 & 2.40\\
%         Falcon & scidef & 60 & 3.67 & 0.47 & 4.00 & 0.47 & 0.66 & 2.42\\
%         PaLM2 & scidef & 60 & \textbf{17.65} & 0.46 & \textbf{4.42} & 0.46 & 0.60 & 2.43\\
%         GPT4 & scidef & 60 & 4.24 & \textbf{0.62} & 4.33 & \textbf{0.62} & \textbf{0.84} & 2.50\\
        
%     \bottomrule
%     \end{tabular}
%     \caption{Human evaluations of LLMs generations for concept simplification}
%     \label{tab:h_metrics}
% \end{table*}

% Prompt 1: -- "Simplify the definition.
% Definition: Electron Microscope is an instrument that provides highly magnified images by use of an electron beam".

% Prompt 2 -- "Rewrite the definition simplifying the concept: "magnify". Electron Microscope is an instrument that provides highly magnified images by use of an electron beam".

% Prompt 3 -- "Rewrite the definition integrating an explanation for the concept: magnify. Electron Microscope is an instrument that provides highly magnified images by use of an electron beam".

% Rewrite the definition simplifying the concept: ``magnify.''
        % Definition: Electron Microscope is an instrument that provides highly magnified images by use of an electron beam. \\
% Concept: ``magnify.''
        %     Definition: Electron Microscope is an instrument that provides highly magnified images by use of an electron beam.
        %     Rewrite: Electron Microscope is an instrument that provides highly zoomed in images by use of an electron beam.
        %     Concept: ``liberty.''
        %     Definition: Liberalism is a political philosophy or worldview founded on ideas of liberty and equality.
        %     Rewrite:\\
        
% Rewrite the definition integrating an explanation for the concept: ``magnify.''
        % Definition: Electron Microscope is an instrument that provides highly magnified images by use of an electron beam.
        % Rewrite: \\

% add-context-3-shot & Concept: ``magnify.''
        %     Definition: Electron Microscope is an instrument that provides highly magnified images by use of an electron beam.
        %     Rewrite: Electron Microscope is an instrument that provides highly magnified images by use of an electron beam. Magnification is looking at an enlarged version of the object.
        %     Concept: ``liberty.''
        %     Definition: Liberalism is a political philosophy or worldview founded on ideas of liberty and equality.
        %     Rewrite:\\
        
% Suggestion: In the modeling section you should introduce variable names to correspond to these things, for example: $(p, d_o)$ = phrase, its corresponding definition $c$ = $d^{i...j}_o$ = difficult concept consisting of sequence of words found in the definition $d_r$ = rewritten definition. That way you can have an easier way of referring to these throughout the paper, e.g. here you could just say that you show the model inputs (p, d_o, c) and output (d_r)

% %If a concept is important in a specific domain, we expect it will have a Wikipedia article with the concept name as the title.
%We start with a dataset of Wikipedia articles annotated by topic (domain) assignments~\cite{Johnson2021}.


% Cogsci stuff
% \begin{figure}
%     \centering
%     %\includegraphics[width=\linewidth]{latex/figures/text_difficulty_overview.png}
%     \includegraphics[width=\linewidth]{latex/figures/revised_fig1.png}
%     \caption{Lexical simplification (above) improves readability but also abstracts subject-specific terminologies. Given a difficult concept (e.g., \textit{cerebellum}), conceptual simplification can address reader-specific difficulty in the text while preserving subject-specific terminologies and descriptions (below).}
%     \label{fig:text_difficulty_overview}
% \end{figure}

% During comprehension, relevant schemas (mental frameworks or structures that help organize and interpret information) are activated to help interpret the new information.

% The rationale for the survey questions becomes to understand the increase in understanding from the definitions.

% "Photosynthesis is the process by which green plants and some other organisms use sunlight to synthesize foods with the help of chlorophyll, converting carbon dioxide and water into glucose and oxygen."
% If readers do not know synthesize

% Supporting reading comprehension of difficult text requires bridging the gap between their current knowledge and the concepts presented in the text~\citet{graesser1994constructing, dunietz-etal-2020-test}. Text simplification~\citet{siddharthan2006syntactic}, an extensively studied field in NLP, is one approach that supports understanding difficult text by simplifying complex syntax and substituting complex words with simpler alternatives~\citet{kim-etal-2016-simplescience}. However, text simplification also sacrifices important information for simplicity~\citet{garbacea-etal-2021-explainable}.

% Providing readers aids such as such as contextual explanations for complex terms, examples, and analogies can facilitate comprehension without sacrificing information. Research in cognitive science suggests that readers continually integrate information from the text into their world model~\citet{lorch1997understanding, van2010using} and such aids can help in the process. Recent prior work in NLP on providing contextual elaborative explanations of difficult text supports this direction~\cite{wu-etal-2023-elaborative}. \sumit{revisit to add one more argument}


% Successful reading comprehension happens when readers are able to relate the text 
% Successful reading comprehension is key to integration of new knowledge and fostering learning from text~\cite{lorch1997understanding,dunietz-etal-2020-test}. Reading comprehension is shaped by the coherence of text and also reader's comprehension skills,  their background knowledge and reading goals~\cite{van2010using}. Cognitive theories of comprehension suggest that comprehension is a multi-stage process primarily involving 1) local meaning representation of text -- concepts, facts about concepts, and relations between them~\cite{graesser1994constructing}, 2) Constructing a "schema" of the text, and filling in gaps using background knowledge to create a "mental picture" of what the text is about~\cite{bartlett1995remembering, kintsch1978toward}. A "schema" is a mental organization of information to help individuals understand and predict situations or knowledge. Even for skilled adult readers who can build successful local meaning of text, lack of domain knowledge (e.g, concepts, relations between them, processes) can impact comprehension of coherent text. This is because they are unable to create a coherent or complete schema through the use of inferences on their background knowledge. 

%Providing readers aids such as such as contextual explanations for complex concepts, examples, and analogies can provide readers with necessary associations into their background knowledge, to support their schema creation for comprehension. While text simplification supports comprehension by conveying the meaning in simpler terms~\cite{zhang-lapata-2017-sentence}, it does so at the expense of losing important information~\cite{garbacea-etal-2021-explainable}. 

% Such aids, \textit{provided in the service of supporting connection of text to relevant background knowledge}, have been found useful for comprehension both in cognitive science~\cite{graesser1994constructing} and more recently in Machine Reading Comprehension (MRC)~\cite{dunietz-etal-2020-test}, elaborative explanations~\cite{srikanth-li-2021-elaborative}, and commonsense inferences~\cite{omura-etal-2020-method}.

% https://www.tandfonline.com/doi/abs/10.1207/S1532690XCI1804_4
% https://arxiv.org/abs/1305.6360
% https://journals.sagepub.com/doi/abs/10.1177/001872088903100101
% 2LL and comprehension aids - https://www.proquest.com/docview/304997470?pq-origsite=gscholar&fromopenview=true&sourcetype=Dissertations%20&%20Theses
% Audio-visual on foreign language - https://journals.sagepub.com/doi/abs/10.2466/24.PMS.120v14x2
% Reading aids to comprehension - https://www.tandfonline.com/doi/abs/10.1080/00461528409529279

% use the cogsci work on schema creation

%This is because they are unable to create a coherent or complete schema through the use of inferences on their background knowledge.
% ``Schema'' theory was first developed by  ~\citet{bartlett1995remembering} to explain the the distortions, and selective recall of narratives by people based on cultural factors. Since then, cognitive psychology has extensively employed the theory to explain comprehension using background knowledge~\cite{kintsch1991role}, impact of reader goals in comprehension, how textual cues can support comprehension. Schema are mental representations of concepts and relations to organize and interpret information to help make sense of the world. It allows active inference using the text and background knowledge necessary for reader's goals.

% Using lexical dictionaries to substitute complex words with simpler alternatives~\cite{pavlick-callison-burch-2016-simple, deleger-zweigenbaum-2009-extracting}, simplifying complex language syntax~\cite{siddharthan2006syntactic} or neural models~\cite{zhang-lapata-2017-sentence} that generate lower reading-grade level~\cite{xu-etal-2015-problems} text all make it easier for readers to activate schemas that are known to them. 

%Lack of vocabulary and reading comprehension can make it difficult for children and second language learners to infer the knowledge in text~\cite{barnett1986, tan2020task}. Complex syntax such as anaphora or compound sentences can pose grammatical difficulty in integrating information in text in the background schema~\cite{nelson2006}. 
% However, even with sufficient vocabulary, and knowledge of language constructs, readers may find it difficult to integrate domain-specific text due to lack of knowledge of related concepts~\cite{cain1999inference,van2010using} in their memory representations. Explanations, definitions, and examples can help readers overcome this difficulty. While there are studies that explore what reading difficulties specific reading groups may encounter (e.g., autism readers)~\cite{}, there has been no exploration for general-purpose difficulties that even skilled adult readers may face, due to lack of a challenging domain-specific corpus.

% Even many recent approaches in NLP such as Machine Reading Comprehension (MRC)~\cite{dunietz-etal-2020-test}, elaborative explanations~\cite{srikanth-li-2021-elaborative}, commonsense inferences~\cite{omura-etal-2020-method} or discourse comprehension~\cite{tian-etal-2020-scene, li-etal-2020-connecting} provide aids by posing questions and answering them and can be viewed as supporting the connection between schema and background knowledge.

%In our task, we start with a natural language definition $d$, which describes a concept $c \in \mathcal{C}$ in a domain $\mathcal{D}_{i} \in \mathcal{D}$ (e.g., the definition of chiari malformations shown in Figure \ref{fig:text_difficulty_overview}). The definition $d$ is described using a set of other concepts $\{c_1, c_2...c_k\} \in \mathcal{C}$. A reader may be unfamiliar with one or more of the difficult concepts in the definition $[c^d_1, c^d_2...] \in \mathcal{C}$ (e.g., ``cerebellum'') making it difficult to understand the definition $d$. The task input is a tuple of the definition and one or more difficult concepts that are mentioned in the definition $(d, [c^d_1, c^d_2...])$. The task output is a rewritten natural language definition $d'$ that contains aids to support the reader to understand the definition $d'$ even if they did not originally know the difficult concepts $[c^d_1, c^d_2...]$. These aids can be any additional content or rephrasing of original content that helps in comprehension. They can be explanations, examples, analogies, visual or auditory aids as identified in our user study, or any other novel strategies beyond these.

%For example, a layperson who wants to know about the topic ``flower anatomy'' may come across the definition ``panicle'' in Figure~\ref{fig:running_example}. 
% For example, a person who is interested in flowers but doesn't have a background in botany might look up a definition like the one in Figure~\ref{fig:running_example}. 
%Their lack of knowledge about the concept ``inflorescence'' used in the definition can prevent them from fully comprehending the meaning of ``panicle''.
% However, they won't find this definition helpful if they are unfamiliar with the botanical term ``inflorescence.''
%While understanding much of the text, they may struggle with just one or two words, such as ``inflorescence''. 
 % AI tools could help rewrite the text to support understanding ``inflorescence'', for instance by lexically substituting the concept with ``flower cluster'' or by elaborating on the concept.  This is a more \textit{focused} form of simplification towards just the concept ``inflorescence,'' but doesn't necessitate simplifying the rest of the text's reading level. 
 
 % we explore commonly used automatic metrics and find that none of them are robust enough to capture the full range of human judgements, indicating that there's much need for future work towards contextual explanations, and new metrics to measure their effectiveness.

%simplifying the entire text to a lower reading grade~\cite{agrawal-carpuat-2023-controlling}, at the cost of sacrificing important information may lead to oversimplification for knowledgeable readers~\cite{manchego2021,garbacea-etal-2021-explainable}. Adult readers and domain experts can often use their background knowledge to infer important implications from the text given sufficient explanations for unfamiliar concepts.

% Let's say a user wants to know about the topic ``how plants get energy''? 
% Below definition about photosynthesis provides some information.
% % it is unclear how glucose is related to energy.
% \blockquote{\textit{Photosynthesis is the process by which green plants and some other organisms use sunlight to synthesize foods with the help of chlorophyll, converting carbon dioxide and water into glucose and oxygen. }}

% A reader familiar with the concept ``glucose'' can make the following elaborative inference \textit{implicitly} -- \textit{\textcolor{red}{plants get  energy from glucose}}. However, if the reader is unfamiliar with the topic, they would be unable to make the inference. Consequently the following \textit{additional} information about glucose can support an unfamiliar reader about plants' energy source \textit{explicitly}. 

% \blockquote{\textit{\textcolor{blue}{Glucose is a complex sugar that contains energy in its chemical bonds.} -> \textcolor{red}{plants get  energy from glucose}}}

%Let's say a user wants to know about the topic ``flower anatomy''.They come across the following definition ``Panicle'' in this topic that provides some information.
% \blockquote{\textit{A panicle is a much-branched \textcolor{red}{inflorescence}.}}

% A reader familiar with the concept that ``inflorescence describes clusters of flowers'' can make the following elaborative inference \textit{implicitly} to develop a richer understanding about the topic -- \textit{\textcolor{blue}{Panicles have several branches of flowers.}} 

% However, if the reader is unfamiliar with the \difficultconcept ``inflorescence'', they would struggle to develop this rich understanding just from the original definition. Consequently the following \textit{explicit additional} information about ``inflorescence'' can help an unfamiliar reader understand ``Panicles'' better in familiar terms. 

% \blockquote{\textit{\textcolor{black}{Inflorescence describes a cluster of flowers} -> \textcolor{blue}{Panicles have several branches of flowers.}}}

% The additional sentence clarifies that glucose is not just a product of photosynthesis but also serves a critical function in storing energy for plants. 


% Key gaps: 
% 1) Lexical simplification focuses on word substitutions and explanations,
% 2) Focus was on new language learners, dyslexic aphasic readers with everyday text. There's an opportunity to explore what can help lay readers with difficult domain-specific text. Lack a dataset here.
% 3) LLMs can go much beyond simple definitions, and substitutions. We have little knowledge how they do that.
% In this work, we focus on a subset of simplification: controllable simplification of user-specified difficult concepts that help readers utilize their background knowledge to develop a coherent mental representation of the text~\cite{kintsch1991role,van2010using}. Cognitive science theories of comprehension have extensively illustrated that effective comprehension occurs when readers can fill-in relevant missing gaps using their background knowledge to develop a rich understanding~\cite{van2010using}. While lexical simplification has shown evidence for personalized lexeme simplification in special cases (e.g., dyslexic or aphasic readers)~\cite{ziegler2008developmental}, LLMs can go much beyond early systems in simplifying compound domain-specific concepts to help lay readers understand domain-specific text. We have limited knowledge on what factors cause difficulty in comprehension of domain-specific text for lay adult readers of difficult text and how current NLP technologies (e.g., LLMs) can alleviate these difficulties while preserving the parts of the text they are familiar with.

% % In this work, we investigate what difficulties lay readers find in comprehending domain-specific complex text and how to use LLMs to alleviate the salient difficulties. 
% We first collect a challenging dataset of domain 30k specific challenging definitions from Wikipedia spanning 13 domains (e.g., Physics, Biology, Geography). We then conduct a formative study of what difficulty users may find in complex definitions and how they might use an AI tutor to alleviate these difficulties. We find evidence of difficulties arising from difficult concepts, need for clarifications, over-specification, complex syntax that can limit schema creation. We also found that participants looked for aids like explanations for difficult concepts, examples, or analogies and auditory or visual aids that can better support schema creation by aiding their background knowledge.

% To evaluate the use of LLMs for supporting better schema creation for comprehension, we create a task to address the most important difficulties that our participants identified -- simplifications and explanations of difficult concepts. We first develop a heuristic to identify difficult concepts occurring in domain-specific definitions in our \datawiki dataset. We then benchmark four LLMs (two open-source and two commercial) on the task of supporting comprehension through rewriting definitions by simplifying or explaining of difficult concepts. Our human evaluations across 2880 original-LLM rewritten definition pairs suggests that LLM rewritten definitions vary significantly in terms of the information that they add, the complexity of the information, and also their ability to successfully alleviate difficulty with the complex concept. 

% Text simplification is a broad domain with different flavors for different target audiences and use-cases. For example, simplifying complex words for language-impaired readers~\cite{paetzold-specia-2016-anita,bingel-etal-2018-lexi}, sentence-level or reading grade-level simplification for children~\cite{agrawal-carpuat-2023-controlling}, or simplifying syntax~\cite{siddharthan2006syntactic}. Parallel corpora from Wikipedia~\cite{kauchak-2013-improving,zhang-lapata-2017-sentence}, or specialized lexicons~\cite{elhadad-sutaria-2007-mining,ong2007simplifying} have advanced simplification research but majority of examples in such datasets are either not challenging for an adult audience (Wikipedia) or too specialized (medicine). \citet{august-etal-2022-generating} created a corpora of scientific definitions from Wikipedia glossaries but they are restricted to a limited number of scientific definitions and do not indicate potentially challenging concepts that may impact comprehension. 

%Facilitating comprehension of technical writing promotes learning and broader communication of ideas.
% Text simplification supports comprehension for students and language learners by substituting complex terms and reducing complex syntax. However, text simplification sacrifices details and specific terminologies necessary for in-depth understanding of challenging subjects. In this work, we propose a new task of supporting the comprehension of technical definitions through concept simplification. We introduce a dataset of about 30,000 definitions spanning thirteen high-level domains extracted from Wikipedia. We evaluate the performance of open-source and commercial LLMs to simplify difficult concepts and introduce a novel concept-graph based metric to evaluate concept simplifications. Our automated and human evaluations suggest that LLMs vary significantly in the amount of changes to address user-specific concept difficulty, meaning preservation ability, and their choice of difficult words. Comparing automated metrics with human evaluations suggests that evaluations using concept graphs capture concept-level changes that existing automated metrics cannot. Automated evaluations and follow-up open-ended human feedback on difficult definitions suggest that users prefer additional context, such as explanations, examples, or illustrations, over simply reducing the reading level of text, opening up new directions for simplification research in NLP.
%Domain specific text can be difficult for lay audience to understand they are unable to build a coherent mental representation that integrates the textual information and relevant background knowledge. TBD.


%Investigations on supporting language-impaired readers (e.g., autism, aphasia)~\cite{paetzold-specia-2016-anita} suggest that that while simplification tends to increase a document's readability, more targeted enhancements (e.g., contextual elaborations) tend to improve text comprehensibility~\cite{rello2013}~\cite{srikanth-li-2021-elaborative}.
% Our task involves simplifying specific words or phrases that may be difficult to understand for readers who are unfamiliar with a given domain, which builds on previous work on identifying and simplifying jargon in text.
% For example, \citet{Guo2023PersonalizedJI} investigate the prediction of individual jargon familiarity, and \citet{august-etal-2022-generating} also generate definitions from concept names, controlling for either a lay audience or a scientific audience.  simplify all complex jargon in a text for a lay audience. 


% Such aids, \textit{provided in the service of supporting connection of text to relevant background knowledge}, have been found useful for comprehension both in cognitive science~\cite{graesser1994constructing}. 


% In NLP, ~\citet{dunietz-etal-2020-test} argued that Machine Reading Comprehension (MRC) can be viewed from the lens of discourse comprehension described as a set of relations between entities and events in the text expressed as a set of questions about them or explicitly modeling them~\cite{tian-etal-2020-scene, li-etal-2020-connecting}. Similarly, ~\citet{srikanth-li-2021-elaborative} studied simplification through elaborations of text, where elaborations explain a part of the text. These approaches can be viewed as supporting the connection of textual information to relevant background schema. 

% Evaluations for simplifications are performed using reading grade-level measures for documents~\cite{heilman-etal-2008-analysis,kincaid1975derivation} or using sentence comparison measures on reference simplification text (e.g., BERTScore)~\cite{bert-score}. The measures include syntax complexity and word-level difficulty, and similarity using embeddings, but they are not sensitive to individual concept-level difficulty.

% While reducing overall text difficulty makes text accessible to students~\cite{mayfield-etal-2019-equity}, lay audience for news consumption~\cite{fatima-strube-2023-cross} or reducing medical jargon difficulty~\cite{joseph-etal-2023-multilingual}, it can negatively affect adults in understanding domain-specific material due to loss of information and subject-specific terminologies~\cite{garbacea-etal-2021-explainable}. Recent survey suggests the lack of  methods to support readers beyond simplifications, such as providing  explanations~\cite{manchego2021}. Even though research suggests difficult concepts can be detrimental to reading comprehension~\cite{kintsch2014reading}, limited prior work has explored how to alleviate difficulty with difficult concepts~\cite{srikanth-li-2021-elaborative}.

% We argue that understanding reading difficulty for skilled readers with unfamiliar domain-specific text can be viewed as supporting construction of relevant schema from text and background knowledge.

One useful application of NLP models is to support people in reading complex texts that may come from unfamiliar domains (e.g., scientific articles). However, existing tools generally simplify or elaborate on the entire text, whereas many human readers may only struggle with one or two concepts in the text. In a preliminary human study, we first identify the salient difficulties that adult readers face with domain-specific text. We then introduce targeted concept simplification, a simplification task for rewriting a piece of text to help a reader understand unfamiliar concepts in the text. We present WikiDomains, a new dataset of 22k definitions from 13 academic domains paired with a difficult concept within each definition. We benchmark how well existing models, including LLMs, perform at this task across human judgment of ease of understanding and meaning preservation. Interestingly, our human judgments preferred eliciting explanations about the difficult concept over asking the LLMs to simplify the concept phrase. However, no model achieves high performance across all quality dimensions, and neither do automated metrics correlate with all human evaluation dimensions, opening up rich avenues for research on personalized human reading comprehension support.

==> reference/correlations_scidef.tex <==
SCIDEF Pearson correlations:
																								
	b1	b2	b3	sentence_bleu	bert_score	graph_similar	aoa	domain	concept_simplified	concept_explained	concept_max	meaning_preservation	change	term_understand	simpler	familiar	rewrite_simpler								
b1	1	0.973	0.935	0.895	0.905	0.475	-0.269	0.106	-0.017	-0.163	-0.102	0.349	0.61	-0.194	0.401	-0.079	-0.374								
b2	0.973	1	0.986	0.961	0.85	0.475	-0.223	0.119	-0.066	-0.112	-0.126	0.356	0.605	-0.185	0.383	-0.097	-0.353								
b3	0.935	0.986	1	0.992	0.791	0.436	-0.188	0.103	-0.095	-0.081	-0.139	0.349	0.593	-0.184	0.369	-0.106	-0.334								
sentence_bleu	0.895	0.961	0.992	1	0.738	0.402	-0.154	0.095	-0.116	-0.06	-0.15	0.343	0.579	-0.181	0.359	-0.101	-0.317								
bert_score	0.905	0.85	0.791	0.738	1	0.569	-0.271	0.156	-0.013	-0.163	-0.097	0.344	0.558	-0.159	0.378	-0.049	-0.341								
graph_similar	0.475	0.475	0.436	0.402	0.569	1	-0.127	0.187	-0.135	-0.044	-0.158	0.236	0.282	-0.066	0.149	-0.08	-0.119								
aoa	-0.269	-0.223	-0.188	-0.154	-0.271	-0.127	1	-0.041	-0.039	0.025	-0.026	-0.122	-0.209	0.037	-0.094	0.115	0.103								
domain	0.106	0.119	0.103	0.095	0.156	0.187	-0.041	1	-0.013	-0.059	-0.044	0.015	0.023	-0.014	0.004	-0.045	-0.045								
concept_simplified	-0.017	-0.066	-0.095	-0.116	-0.013	-0.135	-0.039	-0.013	1	-0.271	0.868	-0.061	-0.023	0.238	-0.065	0.024	0.016								
concept_explained	-0.163	-0.112	-0.081	-0.06	-0.163	-0.044	0.025	-0.059	-0.271	1	0.241	-0.05	-0.154	0.117	-0.113	-0.065	0.159								
concept_max	-0.102	-0.126	-0.139	-0.15	-0.097	-0.158	-0.026	-0.044	0.868	0.241	1	-0.088	-0.103	0.302	-0.124	-0.009	0.097								
meaning_preservation	0.349	0.356	0.349	0.343	0.344	0.236	-0.122	0.015	-0.061	-0.05	-0.088	1	0.553	-0.004	0.378	-0.032	-0.138								
change	0.61	0.605	0.593	0.579	0.558	0.282	-0.209	0.023	-0.023	-0.154	-0.103	0.553	1	-0.148	0.488	-0.098	-0.39								
term_understand	-0.194	-0.185	-0.184	-0.181	-0.159	-0.066	0.037	-0.014	0.238	0.117	0.302	-0.004	-0.148	1	-0.152	0.012	0.294								
simpler	0.401	0.383	0.369	0.359	0.378	0.149	-0.094	0.004	-0.065	-0.113	-0.124	0.378	0.488	-0.152	1	0	-0.478								
familiar	-0.079	-0.097	-0.106	-0.101	-0.049	-0.08	0.115	-0.045	0.024	-0.065	-0.009	-0.032	-0.098	0.012	0	1	0.045								
rewrite_simpler	-0.374	-0.353	-0.334	-0.317	-0.341	-0.119	0.103	-0.045	0.016	0.159	0.097	-0.138	-0.39	0.294	-0.478	0.045	1								
																									
